On the Limits of Tabular Hardness Metrics for Deep RL: A Study with the Pharos Benchmark

Principled evaluation is critical for progress in deep reinforcement learning (RL), yet it lags behind the theory-driven benchmarks of tabular RL. While tabular settings benefit from well-understood hardness measures like MDP diameter and suboptimality gaps, deep RL benchmarks are often chosen based on intuition and popularity. This raises a critical question: can tabular hardness metrics be adapted to guide non-tabular benchmarking? We investigate this question and reveal a fundamental gap. Our primary contribution is demonstrating that the difficulty of non-tabular environments is dominated by a factor that tabular metrics ignore: representation hardness. The same underlying MDP can pose vastly different challenges depending on whether the agent receives state vectors or pixel-based observations. To enable this analysis, we introduce \texttt{pharos}, a new open-source library for principled RL benchmarking that allows for systematic control over both environment structure and agent representations. Our extensive case study using \texttt{pharos} shows that while tabular metrics offer some insight, they are poor predictors of deep RL agent performance on their own. This work highlights the urgent need for new, representation-aware hardness measures and positions \texttt{pharos} as a key tool for developing them.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\RequirePackage{amsmath}        % math utils
\RequirePackage{xspace}         % add the xspace command
\RequirePackage{graphicx}       % to include images
\RequirePackage{csquotes}
\RequirePackage{bbm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

% Custom commands
\newcommand{\vh}[2][]{\ensuremath{\hat v_{#2}(#1)}}
\newcommand{\lrp}[1]{\left(#1\right)}
\newcommand{\lrpq}[1]{\left[#1\right]}

% Math operators
\DeclareMathOperator*{\var}{Var}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Random Variables
\newcommand{\Nrv}[2]{\cN\left(#1,#2\right)}

% Densities
\newcommand{\Nd}[3]{\cN\left(#1;#2,#3\right)}

% Custom variables
\newcommand{\bfw}{\ensuremath{\mathbf{w}}\xspace}

\newcommand{\bA}{\ensuremath{\mathbb A}\xspace}
\newcommand{\bB}{\ensuremath{\mathbb B}\xspace}
\newcommand{\bC}{\ensuremath{\mathbb C}\xspace}
\newcommand{\bD}{\ensuremath{\mathbb D}\xspace}
\newcommand{\bE}{\ensuremath{\mathbb E}\xspace}
\newcommand{\bF}{\ensuremath{\mathbb F}\xspace}
\newcommand{\bG}{\ensuremath{\mathbb G}\xspace}
\newcommand{\bH}{\ensuremath{\mathbb H}\xspace}
\newcommand{\bI}{\ensuremath{\mathbb I}\xspace}
\newcommand{\bJ}{\ensuremath{\mathbb J}\xspace}
\newcommand{\bK}{\ensuremath{\mathbb K}\xspace}
\newcommand{\bL}{\ensuremath{\mathbb L}\xspace}
\newcommand{\bM}{\ensuremath{\mathbb M}\xspace}
\newcommand{\bN}{\ensuremath{\mathbb N}\xspace}
\newcommand{\bO}{\ensuremath{\mathbb O}\xspace}
\newcommand{\bP}{\ensuremath{\mathbb P}\xspace}
\newcommand{\bQ}{\ensuremath{\mathbb Q}\xspace}
\newcommand{\bR}{\ensuremath{\mathbb R}\xspace}
\newcommand{\bS}{\ensuremath{\mathbb S}\xspace}
\newcommand{\bT}{\ensuremath{\mathbb T}\xspace}
\newcommand{\bU}{\ensuremath{\mathbb U}\xspace}
\newcommand{\bV}{\ensuremath{\mathbb V}\xspace}
\newcommand{\bW}{\ensuremath{\mathbb W}\xspace}
\newcommand{\bX}{\ensuremath{\mathbb X}\xspace}
\newcommand{\bY}{\ensuremath{\mathbb Y}\xspace}
\newcommand{\bZ}{\ensuremath{\mathbb Z}\xspace}

\newcommand{\cA}{\ensuremath{\mathcal A}\xspace}
\newcommand{\cB}{\ensuremath{\mathcal B}\xspace}
\newcommand{\cC}{\ensuremath{\mathcal C}\xspace}
\newcommand{\cD}{\ensuremath{\mathcal D}\xspace}
\newcommand{\cE}{\ensuremath{\mathcal E}\xspace}
\newcommand{\cF}{\ensuremath{\mathcal F}\xspace}
\newcommand{\cG}{\ensuremath{\mathcal G}\xspace}
\newcommand{\cH}{\ensuremath{\mathcal H}\xspace}
\newcommand{\cI}{\ensuremath{\mathcal I}\xspace}
\newcommand{\cJ}{\ensuremath{\mathcal J}\xspace}
\newcommand{\cK}{\ensuremath{\mathcal K}\xspace}
\newcommand{\cL}{\ensuremath{\mathcal L}\xspace}
\newcommand{\cM}{\ensuremath{\mathcal M}\xspace}
\newcommand{\cN}{\ensuremath{\mathcal N}\xspace}
\newcommand{\cO}{\ensuremath{\mathcal O}\xspace}
\newcommand{\cP}{\ensuremath{\mathcal P}\xspace}
\newcommand{\cQ}{\ensuremath{\mathcal Q}\xspace}
\newcommand{\cR}{\ensuremath{\mathcal R}\xspace}
\newcommand{\cS}{\ensuremath{\mathcal S}\xspace}
\newcommand{\cT}{\ensuremath{\mathcal T}\xspace}
\newcommand{\cU}{\ensuremath{\mathcal U}\xspace}
\newcommand{\cV}{\ensuremath{\mathcal V}\xspace}
\newcommand{\cW}{\ensuremath{\mathcal W}\xspace}
\newcommand{\cX}{\ensuremath{\mathcal X}\xspace}
\newcommand{\cY}{\ensuremath{\mathcal Y}\xspace}
\newcommand{\cZ}{\ensuremath{\mathcal Z}\xspace}

\newcommand{\tR}{\ensuremath{\text{R}}\xspace}


\newcommand{\bmu}{\ensuremath{\boldsymbol{\mu}}\xspace}
\newcommand{\btheta}{\ensuremath{\boldsymbol{\theta}}\xspace}
\newcommand{\bbeta}{\ensuremath{\boldsymbol{\beta}}\xspace}
\newcommand{\bx}{\ensuremath{\mathbf{x}}\xspace}


% Custom complex commands

% Example of usage: \kl[a][b]
\NewDocumentCommand \kl { o o } {%
  \IfNoValueTF{#2}
   {%
    \IfNoValueTF {#1}
     {%
      \text{KL}\xspace%
     }
     {%
      \text{KL}\xspace%
     }%
   }
   {%
    \text{KL}\lrp{#1\mid\mid#2}%
   }% 
}

% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak



